Magpie: Alignment Data Synthesis from Scratch by Prompting Aligned LLMs with Nothing

High-quality instruction data is critical for aligning large language models (LLMs). Although some models, such as Llama-3-Instruct, have open weights, their alignment data remain private, which hinders the democratization of AI. High human labor costs and a limited, predefined scope for prompting prevent existing open-source data creation methods from scaling effectively, potentially limiting the diversity and quality of public alignment datasets. Is it possible to synthesize high-quality instruction data at scale by extracting it directly from an aligned LLM? We present a self-synthesis method for generating large-scale alignment data named Magpie. Our key observation is that aligned LLMs like Llama-3-Instruct can generate a user query when we input only the left-side templates up to the position reserved for user messages, thanks to their auto-regressive nature. We use this method to prompt Llama-3-Instruct and generate 4 million instructions along with their corresponding responses. We perform a comprehensive analysis of the extracted data and select 300K high-quality instances. To compare Magpie data with other public instruction datasets, we fine-tune Llama-3-8B-Base with each dataset and evaluate the performance of the fine-tuned models. Our results indicate that in some tasks, models fine-tuned with Magpie perform comparably to the official Llama-3-8B-Instruct, despite the latter being enhanced with 10 million data points through supervised fine-tuning (SFT) and subsequent feedback learning. We also show that using Magpie solely for SFT can surpass the performance of previous public datasets utilized for both SFT and preference optimization, such as direct preference optimization with UltraFeedback. This advantage is evident on alignment benchmarks such as AlpacaEval, ArenaHard, and WildBench.

==> motivation.tex <==
\section{Supervision from strong models may not improve SLMs}

In this section, we report a counter-intuitive finding drawn from our extensive experiments:\\
\makebox[\textwidth]{\emph{Supervision from strong models may not improve SLMs.}}
In what follows, we first describe our experimental setup.
We next demonstrate the performance of SLMs fine-tuned with SFT datasets generated by more powerful LLMs.

\subsection{Experimental Setup}

\paragraph{Base SLMs.}
We consider three base SLMs from different developers of varying sizes, including Qwen2-1.5B \citep{qwen2}, Gemma2-2B \citep{gemma_2024}, and Minitron-4B \citep{minitron2024}.

\paragraph{Strong Models for Supervision.}
We use a broad range of models, collectively referred to as \emph{strong models}, to generate SFT datasets to fine-tune each base SLM.
Our strong models include Qwen2 (1.5B, 7B, and 72B) \citep{qwen2}, Llama3 (8B and 70B) \citep{dubey2024llama}, Llama3.1 (8B, 70B, and 405B) \citep{llama31}, and Gemma2 (2B, 9B, and 27B) \citep{team2024gemma}.

\paragraph{Datasets.}

\paragraph{Evaluation Benchmarks.} 
We evaluate the performance of fine-tuned SLMs using two benchmarks: AlpacaEval 2 \citep{alpaca_eval} (referred to as AE 2) and Arena-Hard \citep{arenahard2024} (referred to as AH).
Specifically, AE 2 contains 805 representative instructions from real user interactions. 
AH contains 500 challenging user queries. 
AE 2 and Arena-Hard use GPT-4 Preview and GPT-4-0314 as the baselines to assess the performance of fine-tuned SLMs, respectively.
Both benchmarks compare responses generated by the model of interest with those generated by baselines, and employ GPT evaluators to automatically annotate which response is preferred.

\paragraph{Evaluation Metrics.} 
Similar to existing studies, we adopt two metrics to measure the performance of fine-tuned SLMs.
The first metric, used by both benchmarks, is the \textbf{win rate (WR)}, which calculates the fraction of responses that are favored by the GPT evaluator.
The second metric, used by AlpacaEval 2 benchmark, is the \textbf{length-controlled win rate (LC)} \cite{dubois2024length}.
LC accounts for response length to reduce its impact on WR.

\textbf{Additional Details on Experimental Setups.} Fine-tuing hyper-parameters, hardware, etc can be found in Appendix.

\subsection{Key Findings on Fine-Tuning SLMs with Strong Supervision}

\begin{table*}[tb]\renewcommand{\arraystretch}{0.9} 
\small
% \vspace{0.5mm}
	\centering
	\caption{\small SLM. } 
\setlength{\tabcolsep}{0.4mm}
\resizebox{\textwidth}{!}{
\begin{tabular}{cccccccccccccccc}
    \toprule
 \multirow{3}{*}{Base SLM} & \multirow{3}{*}{Metric} &  \multicolumn{14}{c}{Strong Models} \\ \cmidrule{3-16}
 & & & Qwen2 & & & & Llama3 & & & Llama3.1 & & & & Gemma &\\ \cmidrule{3-5} \cmidrule{7-8} \cmidrule{10-12} \cmidrule{14-16}
 & & 1.5B & 7B & 72B & & 8B & 70B & & 8B & 70B & 405B & & 2B & 9B & 27B \\ 
\midrule
\multirow{3}{*}{Qwen2-1.5B} & AE 2 WR & 0.92 &4.2 &2.14 & &2.32 &3.42 & &1.94 &2.54 &2.16 & &5.49 &4.82 &5.19\\
 & AE 2 LC & 0.62 & 3.21 & 1.29 &  & 1.43 & 2.24 & & 1.02 &1.58 &1.31 & &3.94 &3.51 &3.77\\
 & AH & 0.4 &3.2 &1.3 & &1.4 &1.5 & &1.4 &2.3 &1.8 & &4 &3.1 &3.5\\
 \midrule
 \multirow{3}{*}{Gemma2-2B} & AE 2 WR & 1.69 &8.15 &5.25 & &5.94 &8.29 & &6.53 &7.29 &8.07 & &17.18 &14.06 &13.22\\
 & AE 2 LC & 1 &6.49 &4.03 & &4.18 &6.19 & &4.87 &5.14 &5.68 & &13.78 &12.04 &11.01\\
 & AH & 0.3 &6.3 &3.4 & &3.5 &4.5 & &4.2 &4.5 &4.5 & &11.3 &8.3 &7.6\\
\midrule
\multirow{3}{*}{Minitron-4B} & AE 2 WR & 1.24 &7.46 &4.59 & &6.11 &7.38 & &5.94 &6.69 &5.9 & &10.52 &13.65 &11.49\\
 & AE 2 LC & 0.65 &6.13 &3.46 & &4.8 &5.7 & &4.58 &5.27 &4.32 & &8.82 &11.73 &9.82\\
 & AH &0.3 &6.3 &3.8 &  &4.7 &4.8 & &4.2 &4.3 &4.1 & &8.9 &9.6 &8.5\\
\bottomrule
\end{tabular}
}
\label{exp-comparision-IID-setting}
\end{table*}

==> sections/06-limitations.tex <==
\section{Limitations}

==> sections/acknowledgements.tex <==
\subsubsection*{Acknowledgments}



==> tables/attack_prompt.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{r l}\toprule
        \textbf{User:} &  \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} \\
               & How are you \colorbox{green!20}{<|eot\_id|>} \\
           \textbf{Model:} & \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} \\
         & I am doing well! \colorbox{green!20}{<|eot\_id|>} \\ \bottomrule

    \end{tabular}
    \caption{Llama-3-Instruct style conventional message : \colorbox{green!20}{<|eot\_id|>} is $c^e$ control token, while $c^b = \phi$ for Llama-3-Instruct. \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} and  \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} are $c^r$ control tokens, indicating the message is from user or model respectively. \yuchen{a similar suggestion as in Fig~\ref{fig: tsne-synthetic} --- use the spaace more efficiently; we can do it later though} }
    \label{tab:llama3-example}
\end{table}

==> tables/chat-template-llama3.tex <==
% \begin{wraptable}{r}{5.5cm}
\begin{table}[]
    \centering
    \resizebox{0.7\textwidth}{!}{
    % \begin{tabular}{c r l}\toprule
    %   \multirow{4}[4]{*}{Round 1}  & \textbf{User:} &  \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} \\
    %       &     & How are you \colorbox{green!20}{<|eot\_id|>} \\ \cmidrule(lr){2-3}
    %       &  \textbf{Model:} & \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} \\
    %     & & I am doing well! \colorbox{green!20}{<|eot\_id|>} \\ \midrule
    %    \multirow{4}[4]{*}{Round 2}  &   \textbf{User:} &  \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} \\
    %         &   & I'm doing well too. What's the weather like today? \colorbox{green!20}{<|eot\_id|>} \\ \cmidrule(lr){2-3}
    %      &  \textbf{Model:} & \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} \\
    %     & & I’m not sure about the current weather. Would you like me to look it up for you? \colorbox{green!20}{<|eot\_id|>} \\ 
    %      \bottomrule
    % \end{tabular}
    % }

    \begin{tabular}{c r l}\toprule
      \multirow{2}{*}{Step 1}& \textbf{Input:}&  \textcolor{blue!30}{<|start\_header\_id|>user<|end\_header\_id|>}\\ \cmidrule(lr){2-3}
          &  Model Output:   & How are you \textcolor{blue!30}{<|eot\_id|>} \\ \midrule
          \multirow{4}[3]{*}{Step 2}& \textbf{Input:}&  \textcolor{blue!30}{<|start\_header\_id|>user<|end\_header\_id|>}\\
          &     & How are you \textcolor{blue!30}{<|eot\_id|>} \\ 
          &   & \textcolor{blue!30}{<|start\_header\_id|>assistant<|end\_header\_id|>} \\ \cmidrule(lr){2-3}
        & Model Output: & I am doing well! \textcolor{blue!30}{<|eot\_id|>} \\ %\midrule
       % \multirow{4}[4]{*}{Round 2}  &   \textbf{User:} &  \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} \\
       %      &   & I'm doing well too. What's the weather like today? \colorbox{green!20}{<|eot\_id|>} \\ \cmidrule(lr){2-3}
       %   &  \textbf{Model:} & \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} \\
       %  & & I’m not sure about the current weather. Would you like me to look it up for you? \colorbox{green!20}{<|eot\_id|>} \\ 
         \bottomrule
    \end{tabular}
    }
    \caption{Llama-3-Instruct style conventional message : \colorbox{green!20}{<|eot\_id|>} is $c^e$ control token, while $c^b = \phi$ for Llama-3-Instruct. \colorbox{blue!10}{<|start\_header\_id|>user<|end\_header\_id|>} and  \colorbox{blue!10}{<|start\_header\_id|>assistant<|end\_header\_id|>} are $c^r$ control tokens, indicating the message is from user or model respectively. \yuchen{a similar suggestion as in Fig~\ref{fig: tsne-synthetic} --- use the spaace more efficiently; we can do it later though} 
    \yuchen{we'll need to refine the figure to ensure that general readers can understand our approach by solely looking at this figure/table + captions. the current version is a bit hard to follow.  It seems that this table/figure is only serving to let people understand the Llama-3-instruct's template. it'd be much better if we can use the space more efficiently and also highlight how our method is motivated and done.}
    % \yuchen{to achieve this, we can }
    }
    \label{tab:llama3-example}
\end{table}
% \end{wraptable} 
